ViFi-ReID: A Two-Stream Vision-WiFi Multimodal Approach for Person Re-identification

Person re-identification(ReID), as a crucial technology in the field of security, plays a vital role in safety inspections, personnel counting, and more. Most current ReID approaches primarily extract features from images, which are easily affected by objective conditions such as clothing changes and occlusions. In addition to cameras, we leverage widely available routers as sensing devices by capturing gait information from pedestrians through the Channel State Information (CSI) in WiFi signals and contribute a multimodal dataset. We employ a two-stream network to separately process video understanding and signal analysis tasks, and conduct multi-modal fusion and contrastive learning on pedestrian video and WiFi data. Extensive experiments in real-world scenarios demonstrate that our method effectively uncovers the correlations between heterogeneous data, bridges the gap between visual and signal modalities, significantly expands the sensing range, and improves ReID accuracy across multiple sensors.

==> tables/table1.tex <==
% 消融实验。验证时频结合、数据增强和先进损失函数对最终指标的影响
\begin{table}[htbp]
\centering
\caption{Verifying the impact of data augmentation and advanced losses on each metric.}
\label{table:1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
\multicolumn{3}{c}{Methods} & \multirow{2}{*}{mAP$\uparrow$} & \multirow{2}{*}{mINP$\uparrow$} & \multirow{2}{*}{Rank-1$\uparrow$} & \multirow{2}{*}{Rank-3$\uparrow$} \\
\cline{1-3}
                       Aug. & Sof./Tri. & LMCL/Cro. &                                   &                                   &                                   &        \\
\hline
                       - & Tri. & Cro. & 90.05 & 74.58 & 95.33 & 99.07  \\
                       \checkmark & Tri. & Cro. & 91.21 & 75.81 & \textbf{98.13} & \textbf{100.00} \\
                       \checkmark & \textbf{Sof.} & Cro. & 89.68  & 82.12 & 94.39 & 96.26 \\
                       \checkmark & Tri. & \textbf{LMCL} & 92.42 & 79.15 & \textbf{98.13} & 99.07 \\
                       - & \textbf{Sof.} & \textbf{LMCL} & 91.41 & 83.39 & 96.26 & 99.07  \\
                       \checkmark & \textbf{Sof.} & \textbf{LMCL} & \textbf{93.68} & \textbf{85.19} & \textbf{98.13} & \textbf{100.00}  \\
\hline
\end{tabular}%
}
\vspace{-.35cm}
\end{table}


==> tables/table2.tex <==
% 不同特征融合方法的对比
\begin{table}[htbp]
\centering
\caption{Comparison of different feature fusion methods.}
\label{table:2}
\begin{tabular}{ccccc}
\hline
Fusion & mAP$\uparrow$ & mINP$\uparrow$ & Rank-1$\uparrow$ & Rank-5$\uparrow$ \\
\hline
Early Fusion & 93.45 & 82.70 & 97.20 & 99.07 \\
Late Fusion & 92.54 & 84.01 & \textbf{98.13} & \textbf{100.00} \\
CLS (Ours) & \textbf{93.68} & \textbf{85.19} & \textbf{98.13} & \textbf{100.00} \\
\hline
\end{tabular}
\vspace{-.35cm}
\end{table}


==> tables/table3.tex <==
% 不同网络模型的对比
\begin{table}[htbp]
\centering
\caption{Comparison of different network models.}
\label{table:3}
\begin{tabular}{ccccc}
\hline
Method & mAP$\uparrow$ & mINP$\uparrow$ & Rank-1$\uparrow$ & Rank-5$\uparrow$ \\
\hline
MobileNetv3\cite{9008835} & 85.45 & 75.20 & 91.30 & 94.07 \\
ResNet\cite{he2016deep} & 90.54 & 80.01 & 95.13 & 98.00 \\
ResNext\cite{xie2017aggregated} & 91.10 & 81.00 & 96.20 & 98.60 \\
ShuffleNet\cite{8578814} & 89.80 & 79.50 & 94.70 & 97.30 \\
LSTM\cite{shi2015convolutional} & 87.60 & 77.80 & 92.80 & 95.50 \\
Ours & \textbf{93.68} & \textbf{85.19} & \textbf{98.13} & \textbf{100.00} \\
\hline
\end{tabular}
\vspace{-.35cm}
\end{table}

